Strategic Abilities of Asynchronous Agents: Semantic Side Effects and How to Tame Them

Recently, we have proposed a framework for verification of agents' abilities in asynchronous multi-agent systems, together with an algorithm for automated reduction of models. The semantics was built on the modeling tradition of distributed systems. As we show here, this can sometimes lead to counterintuitive interpretation of formulas when reasoning about the outcome of strategies. First, the semantics disregards finite paths, and thus yields unnatural evaluation of strategies with deadlocks. Secondly, the semantic representations do not allow to capture the asymmetry between proactive agents and the recipients of their choices. We propose how to avoid the problems by a suitable extension of the representations and change of the execution semantics for asynchronous MAS. We also prove that the model reduction scheme still works in the modified framework.

==> coercer-model-v5.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=1cm]
\tikzstyle{epsilontrans}=[draw=grey,dotted line]

\node[state] (s0) {$q_0^c$};
\node[state] (sgva) [label={$\prop{revealed_{\voterno,\prop{a}}}$}, left=1.5cm of s0] 	{$q_{\voterno,\prop{a}}^c$};
\node[state] (sgvb) [label={$\prop{revealed_{\voterno,\prop{b}}}$}, right=1.5cm of s0] 	{$q_{\voterno,\prop{b}}^c$};

\node[state] (s1) [below left=2.5cm and 0.75cm of s0]	{$q_{s,\voterno}^c$};
\node[state] (s2) [label=below:{$\prop{punished_\voterno}$}, below right=2.5cm and 0.75cm of s0]	{$q_{p,\voterno}^c$};

\path
(s0)
	edge [bend left=20]			node [sloped, anchor=center, above] 	{$gv_{\voterno,\prop{a}}$}	(sgva)
	edge [bend right=20]			node [sloped, anchor=center, above] 	{$gv_{\voterno,\prop{b}}$}	(sgvb)
	edge [loop above]			node [above=0.2cm] 	{$ng_\voterno$}	(s0)
	edge [bend left=20]		node [sloped, anchor=center, above]		{$stop_\voterno$}		(s1)
(s1)
	edge [bend left=20]		node [sloped, anchor=center, above] 	{$return$}	(s0)
	edge	node [sloped, anchor=center, above]		{$pun_\voterno$}	(s2)
(s2)
	edge [bend right=20] 	node [sloped, anchor=center, above]		{$return$}	(s0)
(sgva)
	edge [bend left=20] 	node [sloped, anchor=center, above]		{$return$}	(s0)
(sgvb)
	edge [bend right=20] 	node [sloped, anchor=center, above]		{$return$}	(s0);


==> conference-gc.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{privlabel}=[text=\private]
\tikzstyle{privtrans}=[draw=\private]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[state] (s1) [below of=s0, label=above left:{\large $\prop{open}$}] {$1$};
\node[state] (s2) [below left=1cm and 0.6cm of s1] {$2$};
\node[state] (s3) [below right=1cm and 0.6cm of s1] {$3$};

\path
(s0)
  edge [loop left,privtrans] node[privlabel,midway,above=5pt] {$prepare$} (s0)
  edge node[near start,right] {${proceed}$}	(s1)
(s1)
  edge node[near start,left] {${onsite}$} (s2)
  edge node[near start,right] {${online}$} (s3)
(s2)
  edge [loop below,privtrans] node[privlabel,midway,below] {$rest$} (s2)
(s3)
  edge [loop below,privtrans] node[privlabel,midway,below] {$rest$} (s3);


==> conference-oc+strat.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{privlabel}=[]
\tikzstyle{privtrans}=[]
\tikzstyle{strat}=[very thick]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[state] (s1) [below left=1.4cm and 0.6cm of s0, label=above:{\large $\prop{epid}\quad{}$}] {$1$};
\node[state] (s2) [below right=1.4cm and 0.6cm of s0] {$2$};

\path
(s0)
%  edge [loop left] node[midway, left] {$\mathbf{a}$} (s0)
  edge node[near start,left] {$onsite$} (s1)
  edge[strat] node[near start,right] {$online$}	(s2)
(s1)
  edge [strat,privtrans,loop below] node[privlabel,midway,below] {$handle$} (s1)
(s2)
  edge [strat,privtrans,loop below] node[privlabel,midway,below] {$handle$} (s2);


==> conference-oc-2.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{privlabel}=[text=\private]
\tikzstyle{privtrans}=[draw=\private]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[state] (s1) [below left=1.4cm and 0.6cm of s0, label=above:{\large $\prop{epid}\quad{}$}] {$1$};
\node[state] (s2) [below right=1.4cm and 0.6cm of s0] {$2$};
\node[state] (s3) [below right=1.2cm and 0.6cm of s1, label=right:{\large $\prop{closed}\quad{}$}] {$3$};

\path
(s0)
%  edge [loop left] node[midway, left] {$\mathbf{a}$} (s0)
  edge node[near start,left] {$onsite$} (s1)
  edge node[near start,right] {$online$}	(s2)
(s1)
  edge [privtrans] node[privlabel,midway,left=-10pt] {$handle$} (s3)
(s2)
  edge [privtrans] node[privlabel,midway,right=-10pt] {$handle$} (s3)
(s3)
  edge [privtrans,loop below] node[privlabel,midway,below] {$idle$} (s3);


==> conference-oc.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{privlabel}=[text=\private]
\tikzstyle{privtrans}=[draw=\private]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[state] (s1) [below left=1.4cm and 0.6cm of s0, label=above:{\large $\prop{epid}\quad{}$}] {$1$};
\node[state] (s2) [below right=1.4cm and 0.6cm of s0] {$2$};

\path
(s0)
%  edge [loop left] node[midway, left] {$\mathbf{a}$} (s0)
  edge node[near start,left] {$onsite$} (s1)
  edge node[near start,right] {$online$}	(s2)
(s1)
  edge [privtrans,loop below] node[privlabel,midway,below] {$handle$} (s1)
(s2)
  edge [privtrans,loop below] node[privlabel,midway,below] {$handle$} (s2);


==> conference-sc.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{privlabel}=[text=\private]
\tikzstyle{privtrans}=[draw=\private]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[state] (s1) [below left=1.4cm and 0.6cm of s0] {$1$};
\node[state] (s2) [below right=1.4cm and 0.6cm of s0] {$2$};

\path
(s0)
  edge node[near start,left] {${proceed}$} (s1)
  edge[privtrans] node[privlabel,near start,right] {$giveup$}	(s2)
(s1)
  edge[loop below] node[midway,below] {$proceed$} (s1)
(s2)
  edge[loop below,privtrans] node[privlabel,midway,below] {$giveup$} (s2);


==> conference-unfolding+strat.tex <==
\tikzstyle{state}=[circle,fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{reachstate}=[state,very thick]
\tikzstyle{strat}=[very thick]

\node[reachstate] (s000) {$000$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[reachstate] (s101) [below of=s000, label=above left:{\large $\prop{open}$}] {$101$};
\node[reachstate] (s002) [right of=s101] {$002$};
\node[state] (s211) [below left=1.4cm and 0.6cm of s101, label=above:{\large $\prop{epid}\quad{}$}] {$211$};
\node[state] (s321) [below right=1.4cm and 0.6cm of s101] {$321$};

\path
(s000)
  %edge [loop left] node[midway,above=5pt] {$prepare$} (s000)
  edge[strat] node[near start, left] {$proceed$}	(s101)
  edge[strat] node[near start, right] {$giveup$} (s002)
(s101)
  edge node[midway, above] {$onsite$}	(s211)
  edge node[midway, above] {$online$}	(s321)
(s002)
  edge[strat,loop below] node[midway,below]{$giveup$} (s002)
(s211)
  edge [loop below] node[midway,below]{$rest$} node[midway,below=10pt]{$handle$} (s211)
(s321)
  edge [loop below] node[midway,below]{$rest$} node[midway,below=10pt]{$handle$} (s321);


==> conference-unfolding.tex <==
\tikzstyle{state}=[circle,fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{reachstate}=[state,very thick]

\node[state] (s000) {$000$}; %[label={[label distance=3.1cm]90:Coercer}];
\node[state] (s101) [below of=s000, label=above left:{\large $\prop{open}$}] {$101$};
\node[state] (s002) [right of=s101] {$002$};
\node[state] (s211) [below left=1.4cm and 0.6cm of s101, label=above:{\large $\prop{epid}\quad{}$}] {$211$};
\node[state] (s321) [below right=1.4cm and 0.6cm of s101] {$321$};

\path
(s000)
  edge [loop left] node[midway,above=5pt] {$prepare$} (s000)
  edge[] node[near start, left] {$proceed$}	(s101)
  edge[] node[near start, right] {$giveup$} (s002)
(s101)
  edge node[midway, above] {$onsite$}	(s211)
  edge node[midway, above] {$online$}	(s321)
(s002)
  edge[loop below] node[midway,below]{$giveup$} (s002)
(s211)
  edge [loop below] node[midway,below]{$rest$} node[midway,below=10pt]{$handle$} (s211)
(s321)
  edge [loop below] node[midway,below]{$rest$} node[midway,below=10pt]{$handle$} (s321);


==> iis-coercion-part.tex <==
%\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=1cm]
\newcommand{\epsGrey}{$\epsilon$}
%\newcommand{\epsGrey}{\color{grey}$\epsilon$}
	
	\node[emph] (s0) {$q_0^1$\\$q_0^2$\\$q_0^c$}; %[label={[label distance=0.0cm]90:Voter $i$}]
  \node[emph] (s1) [below of=s0, xshift=-6.75cm] {$q_a^1$\\$q_0^2$\\$q_0^c$};
  \node[emph] (s2) [below of=s0, xshift=2.25cm] {$q_b^1$\\$q_0^2$\\$q_0^c$};
	\node[norm] (s3) [below of=s0, xshift=-2.25cm]  {$q_0^1$\\$q_a^2$\\$q_0^c$};
  \node[norm] (s4) [below of=s0, xshift=6.75cm] {$q_0^1$\\$q_b^2$\\$q_0^c$};
	
  \node[norm] (s5) [below of=s0, xshift=-8.25cm, yshift=-6cm]  {$q_{a,g}^1$\\$q_0^2$\\$q_0^c$};
  \node[norm] (s6) [below of=s0, xshift=-6.75cm, yshift=-6cm] {$q_{a,n}^1$\\$q_0^2$\\$q_0^c$};
	\node[norm] (s7) [below of=s0, xshift=3.75cm, yshift=-6cm]  {$q_{b,g}^1$\\$q_0^2$\\$q_0^c$};
  \node[norm] (s8) [below of=s0, xshift=5.25cm, yshift=-6cm] {$q_{b,n}^1$\\$q_0^2$\\$q_0^c$};
	\node[emph] (s9) [below of=s0, xshift=-2.25cm, yshift=-6cm]  {$q_a^1$\\$q_b^2$\\$q_0^c$};
  \node[emph] (s10) [below of=s0, xshift=-0.75cm, yshift=-6cm]  {$q_a^1$\\$q_a^2$\\$q_0^c$};
	\node[emph] (s11) [below of=s0, xshift=0.75cm, yshift=-6cm]  {$q_b^1$\\$q_a^2$\\$q_0^c$};
  \node[emph] (s12) [below of=s0, xshift=2.25cm, yshift=-6cm] {$q_b^1$\\$q_b^2$\\$q_0^c$};
	\node[norm] (s13) [below of=s0, xshift=-3.75cm, yshift=-6cm]  {$q_0^1$\\$q_{a,g}^2$\\$q_0^c$};
  \node[norm] (s14) [below of=s0, xshift=-5.25cm, yshift=-6cm] {$q_0^1$\\$q_{a,n}^2$\\$q_0^c$};
	\node[norm] (s15) [below of=s0, xshift=6.75cm, yshift=-6cm] {$q_0^1$\\$q_{b,g}^2$\\$q_0^c$};
	\node[norm] (s16) [below of=s0, xshift=8.25cm, yshift=-6cm] {$q_0^1$\\$q_{b,n}^2$\\$q_0^c$};
	
	\node[emph] (s9ag) [below of=s0, xshift=-4.5cm, yshift=-12cm] {$q_{a,g}^1$\\$q_b^2$\\$q_{1,a}^c$};
	\node[emph] (s9an) [below of=s0, xshift=-3cm, yshift=-12cm] {$q_{a,n}^1$\\$q_b^2$\\$q_0^c$};
	\node[emph] (s9bn) [below of=s0, xshift=-1.5cm, yshift=-12cm] {$q_a^1$\\$q_{b,n}^2$\\$q_0^c$};
	\node[emph] (s9bg) [below of=s0, xshift=0cm, yshift=-12cm] {$q_a^1$\\$q_{b,g}^2$\\$q_{2,b}^c$};
	
	\node[emph] (s9agr) [below of=s0, xshift=-7.5cm, yshift=-12.5cm] {$q_{a,g}^1$\\$q_b^2$\\$q_0^c$};
	\node[emph] (s9bgr) [below of=s0, xshift=3cm, yshift=-12.5cm] {$q_a^1$\\$q_{b,g}^2$\\$q_0^c$};
	
	\node[emph] (s9ags) [below of=s0, xshift=-7.5cm, yshift=-18.5cm] {$q_{a,s}^1$\\$q_b^2$\\$q_{s,1}^c$};
	\node[emph] (s9agbg) [below of=s0, xshift=-6cm, yshift=-18.5cm] {$q_{a,g}^1$\\$q_{b,g}^2$\\$q_0^c$};
	\node[emph] (s9agbn) [below of=s0, xshift=-4.5cm, yshift=-18.5cm] {$q_{a,g}^1$\\$q_{b,n}^2$\\$q_0^c$};
	\node[emph] (s9ans) [below of=s0, xshift=-3cm, yshift=-18.5cm] {$q_{a,s}^1$\\$q_b^2$\\$q_{s,1}^c$};
	\node[emph] (s9anbg) [below of=s0, xshift=-1.5cm, yshift=-18.5cm] {$q_{a,n}^1$\\$q_{b,g}^2$\\$q_0^c$};
	\node[emph] (s9anbn) [below of=s0, xshift=0cm, yshift=-18.5cm] {$q_{a,n}^1$\\$q_{b,n}^2$\\$q_0^c$};
	\node[emph] (s9bns) [below of=s0, xshift=1.5cm, yshift=-18.5cm] {$q_a^1$\\$q_{b,s}^2$\\$q_{s,2}^c$};
	%\node[emph] (s9bnag) [below of=s0, xshift=2.25cm, yshift=-18.5cm] {$q_{a,g}^1$\\$q_{b,n}^2$\\$q_0^c$};
	%\node[emph] (s9bnan) [below of=s0, xshift=3.75cm, yshift=-18.5cm] {$q_{a,n}^1$\\$q_{b,n}^2$\\$q_0^c$};
	\node[emph] (s9bgs) [below of=s0, xshift=3cm, yshift=-18.5cm] {$q_a^1$\\$q_{b,s}^2$\\$q_{s,2}^c$};
	%\node[emph] (s9bgag) [below of=s0, xshift=6.75cm, yshift=-18.5cm] {$q_{a,g}^1$\\$q_{b,g}^2$\\$q_0^c$};
	%\node[emph] (s9bgan) [below of=s0, xshift=8.25cm, yshift=-18.5cm] {$q_{a,n}^1$\\$q_{b,g}^2$\\$q_0^c$};
	
	% level 6
	
	%\node[emph] (s9agsp) [below of=s0, xshift=-7.5cm, yshift=-22cm] {$q_{a,s}^1$\\$q_b^2$\\$q_{p,1}^c$};
	%\node[emph] (s9agsr) [below of=s0, xshift=-6cm, yshift=-22cm] {$q_{a,s}^1$\\$q_b^2$\\$q_0^c$};
	%\node[emph] (s9ansp) [below of=s0, xshift=-4.5cm, yshift=-22cm] {$q_{a,s}^1$\\$q_b^2$\\$q_{p,1}^c$};
	%\node[emph] (s9ansr) [below of=s0, xshift=-3cm, yshift=-22cm] {$q_{a,s}^1$\\$q_b^2$\\$q_0^c$};
	%\node[emph] (s9bnsp) [below of=s0, xshift=-1.5cm, yshift=-22cm] {$q_a^1$\\$q_{b,s}^2$\\$q_{p,2}^c$};
	%\node[emph] (s9bnsr) [below of=s0, xshift=0cm, yshift=-22cm] {$q_a^1$\\$q_{b,s}^2$\\$q_0^c$};
	%\node[emph] (s9bgsp) [below of=s0, xshift=1.5cm, yshift=-22cm] {$q_a^1$\\$q_{b,s}^2$\\$q_{p,2}^c$};
	%\node[emph] (s9bgsr) [below of=s0, xshift=3cm, yshift=-22cm] {$q_a^1$\\$q_{b,s}^2$\\$q_0^c$};
	
		
		
  \path (s0)	edge [emph] 					node [trns, sloped, anchor=center, above] {$vote_{1,a}$} (s1.north)
							edge [emph]       		node [trns, sloped, anchor=center, above] {$vote_{1,b}$} (s2.north)
							edge         					node [trns, sloped, anchor=center, above] {$vote_{2,a}$} (s3.north)
							edge        					node [trns, sloped, anchor=center, above] {$vote_{2,b}$} (s4.north)
							edge [emph,loop below] node[trns] {\epsGrey} (s0)
							
				(s1)	edge         					node [trns, sloped, anchor=center, above, pos=0.5] {$gv_{1,a}$} (s5.north)
							edge        					node [trns, sloped, anchor=center, above, pos=0.5] {$ng_1$} (s6.north)
							edge [emph]        		node [trns, sloped, anchor=center, below, pos=0.33] {$vote_{2,b}$} (s9.north)
							edge [emph]       		node [trns, sloped, anchor=center, above, pos=0.33] {$vote_{2,a}$} (s10.north)
							edge [emph,loop right] node[trns,very near start] {\epsGrey} (s1)
				(s2)	edge        					node [trns, sloped, anchor=center, above, pos=0.5] {$gv_{1,b}$} (s7.north)
							edge        					node [trns, sloped, anchor=center, above, pos=0.4] {$ng_1$} (s8.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.25] {$vote_{2,a}$} (s11.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.6] {$vote_{2,b}$} (s12.north)
							edge [emph,loop left] node[trns,very near end] {\epsGrey} (s2)
				(s3)	edge         					node [trns, sloped, anchor=center, below, pos=0.15] {$gv_{2,a}$} (s13.north)
							edge        					node [trns, sloped, anchor=center, above, pos=0.15] {$ng_2$} (s14.north)
							edge			  					node [trns, sloped, anchor=center, below, pos=0.25] {$vote_{1,a}$} (s10.north)
							edge			  					node [trns, sloped, anchor=center, above, pos=0.25] {$vote_{1,b}$} (s11.north)
							edge [loop right] node[trns,very near start] {\epsGrey} (s3)
				(s4)	edge			  					node [trns, sloped, anchor=center, above, pos=0.15] {$vote_{1,a}$} (s9.north)
							edge			  					node [trns, sloped, anchor=center, below, pos=0.3] {$vote_{1,b}$} (s12.north)
							edge         					node [trns, sloped, anchor=center, below, pos=0.35] {$gv_{2,b}$} (s15.north)
							edge        					node [trns, sloped, anchor=center, above, pos=0.35] {$ng_2$} (s16.north)
							edge [loop left] node[trns,very near end] {\epsGrey} (s4)
				(s5)	edge [loop below] node[trns] {\epsGrey} (s5)
				(s6)	edge [loop below] node[trns] {\epsGrey} (s6)
				(s7)	edge [loop below] node[trns] {\epsGrey} (s7)
				(s8)	edge [loop below] node[trns] {\epsGrey} (s8)
				(s9)	edge [emph,loop below] node[trns] {\epsGrey} (s9)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.66] {$gv_{1,a}$} (s9ag.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.66] {$ng_1$} (s9an.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.66] {$ng_2$} (s9bn.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.66] {$gv_{2,b}$} (s9bg.north)
				(s10)	edge [emph,loop below] node[trns] {\epsGrey} (s10)
				(s11)	edge [emph,loop below] node[trns] {\epsGrey} (s11)
				(s12)	edge [emph,loop below] node[trns] {\epsGrey} (s12)
				(s13)	edge [loop below] node[trns] {\epsGrey} (s13)
				(s14)	edge [loop below] node[trns] {\epsGrey} (s14)
				(s15)	edge [loop below] node[trns] {\epsGrey} (s15)
				(s16)	edge [loop below] node[trns] {\epsGrey} (s16)
				
				(s9ag) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$return$} (s9agr.east)
							 edge [emph,out=150,in=120,looseness=8] node[trns, sloped, anchor=center, above, pos=0.5] {\epsGrey} (s9ag)
				(s9bg) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$return$} (s9bgr.west)
							 edge [emph,out=30,in=60,looseness=8] node[trns, sloped, anchor=center, above, pos=0.5] {\epsGrey} (s9bg)
				
				(s9agr) edge [emph]  					node [trns, sloped, anchor=center, below, pos=0.5] {$stop_1$} (s9ags.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$gv_{2,b}$} (s9agbg.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$ng_2$} (s9agbn.north)
								edge [emph,loop above] node[trns] {\epsGrey} (s9bg)
				(s9an) edge [emph]  					node [trns, sloped, anchor=center, below, pos=0.2] {$stop_1$} (s9ans.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.7] {$gv_{2,b}$} (s9anbg.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.25] {$ng_2$} (s9anbn.north)
								edge [emph,out=130,in=100,looseness=8] node[trns, sloped, anchor=center, below, pos=0.5] {\epsGrey} (s9an)
				(s9bn) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.43] {$stop_2$} (s9bns.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.6] {$gv_{1,a}$} (s9agbn.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$ng_1$} (s9anbn.north)
								edge [emph,out=50,in=80,looseness=8] node[trns, sloped, anchor=center, below, pos=0.5] {\epsGrey} (s9bn)
				(s9bgr) edge [emph]  					node [trns, sloped, anchor=center, below, pos=0.5] {$stop_2$} (s9bgs.north)
								edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.15] {$gv_{1,a}$} (s9agbg.north)
								edge [emph]  					node [trns, sloped, anchor=center, below, pos=0.25] {$ng_1$} (s9anbg.north)
								edge [emph,loop above] node[trns] {\epsGrey} (s9bg)
				
				% level 6
				(s9ags) edge [emph,loop below] node[trns] {\epsGrey} (s9ags)
				(s9agbg) edge [emph,loop below] node[trns] {\epsGrey} (s9agbg)
				(s9agbn) edge [emph,loop below] node[trns] {\epsGrey} (s9agbn)
				(s9ans) edge [emph,loop below] node[trns] {\epsGrey} (s9ans)
				(s9anbg) edge [emph,loop below] node[trns] {\epsGrey} (s9anbg)
				(s9anbn) edge [emph,loop below] node[trns] {\epsGrey} (s9anbn)
				(s9bgs) edge [emph,loop below] node[trns] {\epsGrey} (s9bgs)
				(s9bns) edge [emph,loop below] node[trns] {\epsGrey} (s9bns);
				
				%(s9ags) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$pun_1$} (s9agsp.north)
								%edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$return$} (s9agsr.north)
				%(s9ans) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$pun_1$} (s9ansp.north)
								%edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$return$} (s9ansr.north)
				%(s9bns) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$pun_2$} (s9bnsp.north)
								%edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$return$} (s9bnsr.north)
				%(s9bgs) edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$pun_1$} (s9bgsp.north)
								%edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$return$} (s9bgsr.north);


==> iis.tex <==
	\node[emph] (s0) {$q_0^1$\\$q_0^2$\\$q_0^c$}; %[label={[label distance=0.0cm]90:Voter $i$}]   
  \node[emph] (s1) [below of=s0, xshift=-6.75cm] {$q_a^1$\\$q_0^2$\\$q_0^c$};
  \node[emph] (s2) [below of=s0, xshift=2.25cm] {$q_b^1$\\$q_0^2$\\$q_0^c$};
	\node[norm] (s3) [below of=s0, xshift=-2.25cm]  {$q_0^1$\\$q_a^2$\\$q_0^c$};
  \node[norm] (s4) [below of=s0, xshift=6.75cm] {$q_0^1$\\$q_b^2$\\$q_0^c$};
	
  \node[norm] (s5) [below of=s1, xshift=4.5cm]  {$q_{a,g}^1$\\$q_0^2$\\$q_{g,1,a}^c$};
  \node[norm] (s6) [below of=s1, xshift=6cm] {$q_{a,n}^1$\\$q_0^2$\\$q_{n,1}^c$};
	\node[norm] (s7) [below of=s1, xshift=1.5cm]  {$q_{b,g}^1$\\$q_0^2$\\$q_{g,1,b}^c$};
  \node[norm] (s8) [below of=s3, xshift=-1.5cm] {$q_{b,n}^1$\\$q_0^2$\\$q_{n,1}^c$};
	\node[emph] (s9) [below of=s3, xshift=-6cm]  {$q_a^1$\\$q_b^2$\\$q_0^c$};
  \node[emph] (s10) [below of=s3, xshift=-4.5cm]  {$q_a^1$\\$q_a^2$\\$q_0^c$};
	\node[emph] (s11) [below of=s2, xshift=-1.5cm]  {$q_b^1$\\$q_a^2$\\$q_0^c$};
  \node[emph] (s12) [below of=s2, xshift=0cm] {$q_b^1$\\$q_b^2$\\$q_0^c$};
	\node[norm] (s13) [below of=s2, xshift=1.5cm]  {$q_0^1$\\$q_{a,g}^2$\\$q_{g,2,a}^c$};
  \node[norm] (s14) [below of=s4, xshift=-1.5cm] {$q_0^1$\\$q_{a,n}^2$\\$q_{n,2}^c$};
	\node[norm] (s15) [below of=s4, xshift=0cm] {$q_0^1$\\$q_{b,g}^2$\\$q_{g,2,b}^c$};
	\node[norm] (s16) [below of=s4, xshift=1.5cm] {$q_0^1$\\$q_{b,n}^2$\\$q_{n,2}^c$};
	
	\node[emph] (s29) [below of=s9, xshift=-2.25cm] {$q_{a,g}^1$\\$q_b^2$\\$q_{g,1,a}^c$};
	\node[emph] (s30) [below of=s9, xshift=-0.75cm] {$q_{a,n}^1$\\$q_b^2$\\$q_{n,1}^c$};
	\node[emph] (s31) [below of=s9, xshift=0.75cm] {$q_a^1$\\$q_{b,g}^2$\\$q_{g,2,b}^c$};
	\node[emph] (s32) [below of=s9, xshift=2.25cm] {$q_a^1$\\$q_{b,n}^2$\\$q_{n,2}^c$};
	
	\node[emph] (s29') [below of=s29, xshift=-0.75cm] {$q_0^1$\\$q_b^2$\\$q_{g,1,a}^c$};
	\node[emph] (s29s) [below of=s29, xshift=0.75cm] {$q_{a,g,s}^1$\\$q_b^2$\\$q_{g,1,a}^c$};
	\node[emph] (s29r) [below of=s29, xshift=2.25cm] {$q_{a,g}^1$\\$q_b^2$\\$q_0^c$};
	\node[emph] (s30') [below of=s30, xshift=2.25cm] {$q_0^1$\\$q_b^2$\\$q_{n,1}^c$};
	\node[emph] (s30s) [below of=s30, xshift=3.75cm] {$q_{a,n,s}^1$\\$q_b^2$\\$q_{n,1}^c$};
	\node[emph] (s30r) [below of=s30, xshift=5.25cm] {$q_{a,n}^1$\\$q_b^2$\\$q_0^c$};
	\node[emph] (s31') [below of=s31, xshift=5.25cm] {$q_a^1$\\$q_0^2$\\$q_{g,2,b}^c$};
	\node[emph] (s31s) [below of=s31, xshift=6.75cm] {$q_a^1$\\$q_{b,g,s}^2$\\$q_{g,2,b}^c$};
	\node[emph] (s31r) [below of=s31, xshift=8.25cm] {$q_a^1$\\$q_{b,g}^2$\\$q_0^c$};
	\node[emph] (s32') [below of=s32, xshift=8.25cm] {$q_a^1$\\$q_0^2$\\$q_{n,2}^c$};
	\node[emph] (s32s) [below of=s32, xshift=9.75cm] {$q_a^1$\\$q_{b,n,s}^2$\\$q_{n,2}^c$};
	\node[emph] (s32r) [below of=s32, xshift=11.25cm] {$q_a^1$\\$q_{b,n}^2$\\$q_0^c$};
	
	%\node[norm] (s16a) [below of=s16, xshift=-2.25cm] {$q_a^1$\\$q_{b,ng}^2$\\$q_{ng,2}^c$};
	\node[emph] (s16b) [below of=s16, xshift=-0.75cm] {$q_b^1$\\$q_{b,n}^2$\\$q_{n,2}^c$};
	
	%\node[state] (s9) [label=below:{$voted_{i,B}$}, below of=s5] {$q_{B,g,s}^i$};
	%\node[state] (s10) [label=below:{$voted_{i,B}$}, below of=s6] {$q_{B,n,s}^i$};
	
  \path (s0)	edge [emph] 					node [trns, sloped, anchor=center, above] {$vote_{1,a}$} (s1.north)
							edge [emph]       		node [trns, sloped, anchor=center, above] {$vote_{1,b}$} (s2.north)
							edge         					node [trns, sloped, anchor=center, above] {$vote_{2,a}$} (s3.north)
							edge        					node [trns, sloped, anchor=center, above] {$vote_{2,b}$} (s4.north)
							
				(s1)	edge         					node [trns, sloped, anchor=center, below, pos=0.15] {$gv_{1,a}$} (s5.north) 
							edge        					node [trns, sloped, anchor=center, above, pos=0.15] {$ng_1$} (s6.north) 
							edge [emph]        		node [trns, sloped, anchor=center, above, pos=0.35] {$vote_{2,b}$} (s9.north)
							edge [emph]       		node [trns, sloped, anchor=center, below, pos=0.45] {$vote_{2,a}$} (s10.north)
				(s2)	edge        					node [trns, sloped, anchor=center, above, pos=0.20] {$gv_{1,b}$} (s7.north)
							edge        					node [trns, sloped, anchor=center, below, pos=0.20] {$ng_1$} (s8.north)
							edge [emph]  					node [trns, sloped, anchor=center, below, pos=0.35] {$vote_{2,a}$} (s11.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.45] {$vote_{2,b}$} (s12.north)
				(s3)	edge         					node [trns, sloped, anchor=center, below, pos=0.4] {$gv_{2,a}$} (s13.north)
							edge        					node [trns, sloped, anchor=center, above, pos=0.375] {$ng_2$} (s14.north)
							edge			  					node [trns, sloped, anchor=center, above, pos=0.2] {$vote_{1,a}$} (s10.north east)
							edge			  					node [trns, sloped, anchor=center, below, pos=0.7] {$vote_{1,b}$} (s11.north)
				(s4)	edge			  					node [trns, sloped, anchor=center, above, pos=0.1] {$vote_{1,a}$} (s9.north east)
							edge			  					node [trns, sloped, anchor=center, below, pos=0.3] {$vote_{1,b}$} (s12.north east)
							edge         					node [trns, sloped, anchor=center, below, pos=0.35] {$gv_{2,b}$} (s15.north)
							edge        					node [trns, sloped, anchor=center, above, pos=0.35] {$ng_2$} (s16.north)
							
				(s9)	edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$gv_{1,a}$} (s29.north)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$ng_1$} (s30)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$gv_{2,b}$} (s31)
							edge [emph]  					node [trns, sloped, anchor=center, above, pos=0.5] {$ng_2$} (s32)
				%(s29)	edge [emph, bend left=15]  					node [trns] {$$} (s9.west)
				%(s30)	edge [emph, bend left=15]  					node [trns] {$$} (s9.south west)
				%(s31)	edge [emph, bend right=15]  					node [trns] {$$} (s9.south east)
				%(s32)	edge [emph, bend right=15]  					node [trns] {$$} (s9.east)
				
				(s29)	edge [emph, out=230]  					node [trns, sloped, anchor=center, above] {$repeat_1$} (s29'.north)
							edge [emph, out=250]  					node [trns, sloped, anchor=center, above] {$stop_1$} (s29s.north west)
							edge [emph, out=270]  					node [trns, sloped, anchor=center, above] {$return$} (s29r.north west)
				(s30)	edge [emph, out=240]  					node [trns, sloped, anchor=center, above, pos=0.88, yshift=-5pt] {$repeat_1$} (s30'.north west)
							edge [emph, out=280]  					node [trns, sloped, anchor=center, above, pos=0.92, yshift=-5pt] {$stop_1$} (s30s.north west)
							edge [emph, out=290]  					node [trns, sloped, anchor=center, above] {$return$} (s30r.north west)
				(s31)	edge [emph, out=290]  					node [trns, sloped, anchor=center, above, pos=0.9, yshift=-5pt] {$repeat_2$} (s31'.north west)
							edge [emph, out=300]  					node [trns, sloped, anchor=center, above, pos=0.9, yshift=-5pt] {$stop_2$} (s31s.north west)
							edge [emph, out=310]  					node [trns, sloped, anchor=center, above] {$return$} (s31r.north)
				(s32)	edge [emph, out=350]  					node [trns, sloped, anchor=center, above, pos=0.9, yshift=-5pt] {$repeat_2$} (s32'.north)
							edge [emph, out=10]  					node [trns, sloped, anchor=center, above, pos=0.9, yshift=-5pt] {$stop_2$} (s32s.north)
							edge [emph, out=30]  					node [trns, sloped, anchor=center, above] {$return$} (s32r.north)
							
				(s16)	edge [out=235]			  					node [trns, sloped, anchor=center, above, pos=0.5] {$vote_{1,a}$} (s32.north)
							edge			  					node [trns, sloped, anchor=center, below, pos=0.4] {$vote_{1,b}$} (s16b.north)
							
			  (s12) edge [emph, out=270] 					node [trns, sloped, anchor=center, above, pos=0.375] {$ng_2$} (s16b.north west);
				%(s16a) edge	[out=270, in=0]		  					node [trns, sloped, anchor=center, below, pos=0.4] {$$} (s32.north east);
				%(s16b) edge	[out=255, in=300]		  					node [trns, sloped, anchor=center, below, pos=0.4] {$$} (s12.south);

==> macros.tex <==
% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )

\usepackage{paralist} % for inline lists
\usepackage{stackrel}

% correct bad hyphenation here
% \hyphenation{op-tical net-works semi-conduc-tor}

% BEGIN Watermarking
\ifdefined\VersionWithComments
	\usepackage{draftwatermark}
	\SetWatermarkText{draft}
	\SetWatermarkScale{2}
	\SetWatermarkColor[gray]{0.9}
\fi
% END Watermarking

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\ifdefined\IEEEVersion
%% \newtheorem{assumption}{Assumption}
%%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}
%\newtheorem{example}{Example}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%%\newtheorem{remark}{Remark}
%\newtheorem{theorem}{Theorem}
%\newtheorem{conjecture}{Conjecture}
%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DYNAMIC LINKS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[svgnames,table]{xcolor}
\definecolor{darkgreen}{rgb}{0, 0.5, 0}
\definecolor{darkpurple}{rgb}{0.7, 0, 0.7}
\definecolor{darkblue}{rgb}{0, 0, 0.7}
\definecolor{violetcurie}{RGB}{115,26,67}
\definecolor{forestgreen}{rgb}{0.13,0.54,0.13}

\usepackage[
	colorlinks=true,
	%% \ifdefined\VersionWithComments
	%% 	pagebackref=true,
	%% \fi
        %%MK: somehow breaks things
	citecolor=darkgreen,
	linkcolor=darkblue,
	bookmarksnumbered=true,
	colorlinks=true,
	pageanchor=true,
	urlcolor=darkpurple,
]{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINE NUMBERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[pagewise,switch]{lineno} % switch, modulo, pagewise
	% \linenumbers
	% \renewcommand\linenumberfont{\normalfont\tiny\sffamily\color{gray}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CLEVER REFERENCES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[capitalise,english,nameinlink]{cleveref} % load after algorithm2e and hyperref
	\crefname{line}{\text{line}}{\text{lines}} % to remove the capital

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMENTAIRES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifdefined \VersionWithComments
  \usepackage{marginnote}
%  \usepackage[svgnames]{xcolor}
  \newcommand{\marginX}{\marginnote{\huge{\quad\textbf{!}\quad}}}
  \newcommand{\ea}[1]{\textcolor{purple}{\marginX{}[\textbf{Étienne}: #1]}}
  \newcommand{\mk}[1]{\textcolor{magenta}{\marginX{}[\textbf{Michał}: #1]}}
  \newcommand{\wop}[1]{\textcolor{cyan!75!black}{\marginX{}[\textbf{Wojciech P.}: #1 ]}}
  \newcommand{\wj}[1]{\textcolor{yellow!60!red}{\marginX{}[\textbf{Wojtek J.}: #1
  ]}
 } \newcommand{\lp}[1]{\textcolor{green!70!black}{\marginX{}[\textbf{Laure}: #1 ]}}
  \newcommand{\todo}[1]{\textcolor{red}{\marginX{}TODO: #1}}
  \newcommand{\instructions}[1]{\textcolor{blue}{\marginX{}Instructions: #1}}
\else
  \newcommand{\ea}[1]{}
  \newcommand{\mk}[1]{}
  \newcommand{\wop}[1]{}
  \newcommand{\wj}[1]{}
  \newcommand{\lp}[1]{}
  \newcommand{\todo}[1]{}
  \newcommand{\instructions}[1]{}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DEFINITIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ABBREVIATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\lan}[1]{\textnormal{#1}\xspace}
\newcommand{\CGS}{\lan{CGS}}
\newcommand{\TDCGS}{\lan{TDCGS}}
\newcommand{\PTDCGS}{\lan{PTDCGS}}
\newcommand{\DTS}{\lan{DTS}}
\newcommand{\ATL}{\lan{ATL}}
\newcommand{\ATLstar}{\lan{ATL}^\star}
\newcommand{\TATL}{\lan{TATL}}
\newcommand{\TATLexist}{\exists\TATL\xspace}
\newcommand{\TATLle}{\TATL_{\le, \ge}\xspace}
\newcommand{\TATLeq}{\TATL_{=}\xspace}
\newcommand{\TATLeexist}{\exists\TATLle}
\newcommand{\PTATL}{\lan{PTATL}}
\newcommand{\TATLstar}{\lan{TATL}^\star}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONSTANTS : MATHS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\init}{_0}
\newcommand{\truev}{\top}
\newcommand{\falsev}{\bot}
\newcommand{\grandn}{{\mathbb N}}
\newcommand{\grandnplus}{\grandn_{+}} % \geq 0
\newcommand{\grandq}{{\mathbb Q}}
\newcommand{\grandqplus}{\grandq_{+}} % \geq 0
\newcommand{\grandr}{{\mathbb R}}
\newcommand{\grandrplus}{\grandr_{+}} % \geq 0
\newcommand{\grandz}{{\mathbb Z}}
\newcommand{\Implication}{\ensuremath{\Longrightarrow}}
\newcommand{\mrule}{\;|\;}
\newcommand{\powers}[1]{\mathcal{P}(#1)}
\newcommand{\stcomp}[1]{\overline{#1}}
%\newcommand{\defeq}{\stackrel{def}{=}}
\newcommand{\defeq}{\coloneqq}
\newcommand{\dom}{\mathit{dom}} %domain

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONSTANTS : (T)ATL-specific
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Agents}{\mathit{Agents}}
\newcommand{\agscrd}{{|\Agents|}} %Agents cardinality
\newcommand{\agent}{a}
\newcommand{\propos}{\mathcal{AP}}
\newcommand{\propp}{\mathsf{p}}
\newcommand{\labl}{\mathcal{L}}
\newcommand{\autom}{\mathcal{A}}
\newcommand{\locs}{\mathcal{Q}}
\newcommand{\loc}{q}
\newcommand{\prot}{\ensuremath{\mathit{pr}}}
\newcommand{\gprot}{p}
\newcommand{\outf}{t}
\newcommand{\outm}{\mathcal{E}}
\newcommand{\outcome}{\mathit{out}}
\newcommand{\act}{\mathit{act}}
\newcommand{\actAA}{a}
\newcommand{\actAB}{b}
\newcommand{\actAC}{c}
\newcommand{\actBA}{x}
\newcommand{\actBB}{y}
\newcommand{\actloop}{\iota}
\newcommand{\actions}{\mathit{Act}}
\newcommand{\allactions}{\powers{\actions}\setminus\{\emptyset\}}
\newcommand{\outc}{\mathit{out}}
%% \newcommand{\toatls}[2]{\stackrel[#1]{#2}{\to}}
%% \newcommand{\toatll}[2]{\stackrel[#1]{#2}{\longrightarrow}}
\newcommand{\toatls}[2]{\stackrel{#2,#1}{\to}}
\newcommand{\toatll}[2]{\stackrel{#2,#1}{\longrightarrow}}
\newcommand{\dlangle}[0]{{ \langle\!\langle }}
\newcommand{\drangle}[0]{{ \rangle\!\rangle }}
\newcommand{\blangle}[0]{{ [\![ }}
\newcommand{\brangle}[0]{{ ]\!] }}
\newcommand{\model}{M}
%\newcommand{\model}{\mathcal{M}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\strat}{\sigma}
\newcommand{\Strat}{\Sigma}
\newcommand{\stratcount}{\sigma^{\#}}
\newcommand{\allstratscount}[1]{\Delta^{\#}(#1)}
\newcommand{\strata}{\rho}
\newcommand{\stratb}{\varrho}
\newcommand{\strate}{\varsigma}
\newcommand{\stratf}{\theta}
\newcommand{\stratg}{\vartheta}
\newcommand{\seq}{\pi}
\newcommand{\seqsel}[2]{{#1}(#2)} %element selector
\newcommand{\seqprf}[2]{{#1}_{#2}} %path prefix selector
\newcommand{\seqpostf}[2]{{#1}^{#2}} %path postfix selector
\newcommand{\seqfinalst}[1]{{#1}_F}
\newcommand{\seqmin}[1]{{#1}_{\textnormal{min}}}
\newcommand{\seqminr}[1]{{#1}^R_{\textnormal{min}}}
\newcommand{\tmin}{T_{\textnormal{min}}}
\newcommand{\tmax}{T_{\textnormal{max}}}
\newcommand{\tmaxr}{T^R_{\textnormal{max}}}
\newcommand{\constrval}{\eta}
\newcommand{\getloc}[1]{\mathit{lc}({#1})}
\newcommand{\gettime}[1]{\tau({#1})}
\newcommand{\countmatch}[2]{{\#_{#1}}(#2)}

\newcommand{\modelsY}{\models_Y}
\newcommand{\modelsT}{\models_T}
\newcommand{\modelst}{\models_t}
\newcommand{\modelsr}{\models_r}
\newcommand{\modelsR}{\models_R}
\newcommand{\modelsc}{\models_{\#}}
\newcommand{\modelscnt}[1]{\models_{\#_{#1}}}

\newcommand{\nbAgents}{\ensuremath{m}} % number of agents
% \newcommand{\pr}{x} %parameter
% \newcommand{\params}{\mathcal{X}}
\newcommand{\pr}{\ensuremath{\kappa}} %parameter
\newcommand{\params}{\ensuremath{K}}
\newcommand{\lparams}{\ensuremath{K}_{\mathcal{L}}}
\newcommand{\mparams}{\ensuremath{K}_{\model}}
\newcommand{\pval}{\upsilon}
\newcommand{\pvals}{\mathit{ParVals}}
\newcommand{\parsolutions}[4]{\mathit{MVals}_{#4}(#1, #2, #3)}
\newcommand{\parfsolutions}[4]{\mathit{FVals}_{#4}(#1, #2, #3)}
%
\newcommand{\uconditions}{\mathcal{U}}
\newcommand{\rconditions}{\mathcal{R}}
%
\newcommand{\uconditiona}{\mathcal{U}^{\le\constrval}}
\newcommand{\rconditiona}{\mathcal{R}^{\le\constrval}}
\newcommand{\uconditionb}{\mathcal{U}^{\ge\constrval}}
\newcommand{\rconditionb}{\mathcal{R}^{\ge\constrval}}
\newcommand{\uconditione}{\mathcal{U}^{=\constrval}}
\newcommand{\rconditione}{\mathcal{R}^{=\constrval}}
\newcommand{\stratex}[1]{\widehat{#1}} %extension of a partial strategy
\newcommand{\meet}{\mathit{meet}}
\newcommand{\proofI}{J}
\newcommand{\witness}[1]{\mathit{Wtn}({#1})}
\newcommand{\actpower}[1]{\mathit{AP}({#1})}
\newcommand{\stratsubformulae}[1]{\mathit{SSubFrms}({#1})}
\newcommand{\actpowerrecurs}[1]{\mathit{APO}({#1})}

\newcommand{\nonthreshtdcgs}[1]{\autom_{#1}^{eq}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS FOR ENVIRONMENT ET AL.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\defProblem}[3]
{%	
\noindent\fcolorbox{black}{blue!15}{
	\begin{minipage}{.95\columnwidth}
		\textbf{#1 problem:}\\
		\textsc{Input}: #2\\
		\textsc{Problem}: #3
	\end{minipage}
}
	
	\smallskip
	
}


\newcommand{\recallResult}[2]
{%	
	\smallskip

	\noindent\fcolorbox{black}{green!15}{
		\begin{minipage}{.95\columnwidth}
			\noindent\textbf{\cref{#1} (recalled).}
			{\em{}#2}
		\end{minipage}
	}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% I.E. / E.G. / W.R.T.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Helps to spot the places where macros are NOT used
\ifdefined \VersionWithComments
 	\definecolor{colorok}{RGB}{80,80,150}
\else
	\definecolor{colorok}{RGB}{0,0,0}
\fi

\newcommand{\eg}{\textcolor{colorok}{\textit{e.g.}}\xspace}
\newcommand{\etal}{\textcolor{colorok}{\textit{et al.}}\xspace}
\newcommand{\ie}{\textcolor{colorok}{\textit{i.e.}}\xspace}
\newcommand{\vs}{\textcolor{colorok}{\textit{vs.}}\xspace}
\newcommand{\wrt}{\textcolor{colorok}{w.r.t.}\xspace}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


%%%%%%%%%%%%%%%%%%%%%%%%%%% WJ's macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\prop}[1]{\ensuremath{\mathsf{{#1}}}}
\newcommand{\coop}[2][]{\langle\!\langle{#2}\rangle\!\rangle_{_{\!\mathit{#1}}}}
\newcommand{\Next}[1][]{X_{{#1}}  % Optional parameter: temporal discount
        \,}
\newcommand{\Sometm}[1][]{F_{{#1}}}
\newcommand{\Always}[1][]{G_{{#1}}}
\newcommand{\Until}[1][]{U_{{#1}}}
\newcommand{\WeakUntil}[1][]{W_{{#1}}}
\newcommand{\Release}[1][]{R_{{#1}}}

\newcommand{\srv}{\prop{srv}}
\newcommand{\set}[1]{\{{#1}\}}
\newcommand{\Agt}{{\ensuremath{\mathbb{A}\mathrm{gt}}}}
\renewcommand{\Agents}{\Agt}

  % versions of itemize/enumerate with less vertical spacing
\newenvironment{itemize2}{\begin{itemize}\itemsep 0in}{\end{itemize}}
\newenvironment{enumerate2}{\begin{enumerate}\itemsep 0in}{\end{enumerate}}
\newenvironment{description2}{\begin{description}\itemsep 0in}{\end{description}}

\newcommand{\Mserv}[1][]{\autom_{srv}^{#1}}
\newcommand{\Mservparam}[1][]{\autom_{par}^{#1}}
\newcommand{\wait}{\mathit{wait}}
\newcommand{\req}{\mathit{req}}
\newcommand{\putaway}[1]{}

 % types of strategies
\newcommand{\stratstyle}[1]{\mathrm{#1}}
\newcommand{\tperf}{\stratstyle{T}}
\newcommand{\tmless}{\stratstyle{t}}
\newcommand{\perf}{\stratstyle{R}}
\newcommand{\mless}{\stratstyle{r}}
\newcommand{\cnt}[1][]{\#_{#1}}


==> simplemodel-agent1+strat.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}]  	
  \node (name) [above of=s0] {\Large$\mathbf{1}$};
\node[state] (s1) [below of=s0, label=above left:{\large $\prop{fail}$}] {$1$};
\node[state] (s2) [below left=1cm and 0.6cm of s1] {$2$};
\node[state] (s3) [below right=1cm and 0.6cm of s1] {$3$};

\path
(s0)
  edge[very thick] node[midway, left] {$\mathbf{a}$}	(s1)
(s1)
  edge[very thick] node[midway, above] {$\mathbf{b}$} (s2)
  edge node[midway, above] {$\mathbf{c}$} (s3)
(s2)
  edge [loop below] node[midway, below] {$d$} (s2)
(s3)
  edge [loop below] node[midway, below] {$d$} (s3);


==> simplemodel-agent1.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}]  	
  \node (name) [above of=s0] {\Large$\mathbf{1}$}; 
\node[state] (s1) [below of=s0, label=above left:{\large $\prop{fail}$}] {$1$};
\node[state] (s2) [below left=1cm and 0.6cm of s1] {$2$};
\node[state] (s3) [below right=1cm and 0.6cm of s1] {$3$};

\path
(s0)
  edge node[midway, left] {$\mathbf{a}$}	(s1)
(s1)
  edge node[midway, above] {$\mathbf{b}$} (s2)
  edge node[midway, above] {$\mathbf{c}$} (s3)
(s2)
  edge [loop below] node[midway, below] {$d$} (s2)
(s3)
  edge [loop below] node[midway, below] {$d$} (s3);


==> simplemodel-agent2+strat.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}]  	
  \node (name) [above of=s0] {\Large$\mathbf{2}$};
\node[state] (s1) [below left=1cm and 0.6cm of s0] {$1$};
\node[state] (s2) [below right=1cm and 0.6cm of s0] {$2$};

\path
(s0)
%  edge [loop left] node[midway, left] {$\mathbf{a}$} (s0)
  edge node[midway, above] {$\mathbf{b}$} (s1)
  edge[very thick] node[midway, above] {$\mathbf{c}$}	(s2)
(s1)
  edge [loop below] node[midway, below] {$e$} (s1)
(s2)
  edge [loop below] node[midway, below] {$e$} (s2);


==> simplemodel-agent2.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}]  	
  \node (name) [above of=s0] {\Large$\mathbf{2}$};
\node[state] (s1) [below left=1cm and 0.6cm of s0] {$1$};
\node[state] (s2) [below right=1cm and 0.6cm of s0] {$2$};

\path
(s0)
%  edge [loop left] node[midway, left] {$\mathbf{a}$} (s0)
  edge node[midway, above] {$\mathbf{b}$} (s1)
  edge node[midway, above] {$\mathbf{c}$}	(s2)
(s1)
  edge [loop below] node[midway, below] {$e$} (s1)
(s2)
  edge [loop below] node[midway, below] {$e$} (s2);


==> simplemodel-agent3.tex <==
\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=0.8cm]

\node[state] (s0) {$0$}; %[label={[label distance=3.1cm]90:Coercer}]  	
  \node (name) [above of=s0] {\Large$\mathbf{3}$};
\node[state] (s1) [below left=1cm and 0.6cm of s0] {$1$};
\node[state] (s2) [below right=1cm and 0.6cm of s0] {$2$};

\path
(s0)
%  edge [loop left] node[midway, left] {$\mathbf{a}$} (s0)
  edge node[midway, above] {$\mathbf{a}$} (s1)
  edge node[midway, above] {$f$}	(s2)
(s1)
  edge [loop below] node[midway, below] {$\mathbf{a}$} (s1)
(s2)
  edge [loop below] node[midway, below] {$f$} (s2);


==> simplemodel-unfolding.tex <==
\tikzstyle{state}=[circle,fill=none,draw=black,text=black,minimum size=0.8cm]
\tikzstyle{reachstate}=[state,very thick]

\node[reachstate] (s000) {$000$}; %[label={[label distance=3.1cm]90:Coercer}]  	
  \node (name) [above of=s0] {\Large\textbf{IIS}};
\node[reachstate] (s101) [below of=s000, label=above left:{\large $\prop{fail}$}] {$101$};
\node[reachstate] (s002) [right of=s101] {$002$};
\node[state] (s211) [below left=1.4cm and 0.6cm of s101] {$211$};
\node[state] (s321) [below right=1.4cm and 0.6cm of s101] {$321$};

\path
(s000)
  edge[very thick] node[midway, left] {$\mathbf{a}$}	(s101)
  edge[very thick] node[midway, above] {$f$} (s002)
(s101)
  edge node[midway, above] {$\mathbf{b}$}	(s211)
  edge node[midway, above] {$\mathbf{c}$}	(s321)
(s002)
  edge[very thick,loop below] node[midway, below] {$f$} (s002)
(s211)
  edge [loop below] node[midway, below] {$d,e$} (s211)
(s321)
  edge [loop below] node[midway, below] {$d,e$} (s321);


==> voter-model-v8.tex <==
%% parameterized by the number of the voter: \voterno

\tikzstyle{every state}=[fill=none,draw=black,text=black,minimum size=1cm]

\node[state] (s0)	  {$q_0^\voterno$};

\node[state] (s1) [label={160:{$\prop{voted_{\voterno,\prop{a}}}$}}, below left=1cm and 1.2cm of s0] 	{$q_\prop{a}^\voterno$};
\node[state] (s2) [label={270:{$\prop{voted_{\voterno,\prop{a}}}\qquad{}$}}, below left of=s1]		{$q_{\prop{a},g}^\voterno$};
\node[state] (s3) [label={270:{$\prop{{}\quad\ voted_{\voterno,\prop{a}}}$}}, below right=0.75cm and 0.25cm of s1]	  {$q_{\prop{a},n}^\voterno$};
\node[state] (s4) [label={270:{$\prop{voted_{\voterno,\prop{a}}}$}}, below=2.3cm of s1] {$q_{\prop{a},s}^\voterno$};
%  \node[state] (s5) [label={[label distance=0.0cm]270:{$\prop{voted_{\voterno,\prop{a}}}$}}, below=0.8cm of s3] {$q_{\prop{a},\bar{n}}^\voterno$};

\node[state] (s1bis) [label={20:{$\prop{voted_{\voterno,\prop{b}}}$}}, below right=1cm and 1.2cm of s0] 	{$q_\prop{b}^\voterno$};
\node[state] (s2bis) [label={270:{${}\qquad \prop{voted_{\voterno,\prop{b}}}$}}, below right of=s1bis]		{$q_{\prop{b},g}^\voterno$};
\node[state] (s3bis) [label={270:{$\prop{voted_{\voterno,\prop{b}}}\quad{}$}}, below left=0.75cm and 0.25cm of s1bis]	  {$q_{\prop{b},n}^\voterno$};
\node[state] (s4bis) [label={[label distance=0.0cm]270:{$\prop{voted_{\voterno,\prop{b}}}$}}, below=2.3cm of s1bis] {$q_{\prop{b},s}^\voterno$};
	
\path
(s0)
  edge node[sloped, anchor=center, above] {$vote_{\voterno,\prop{a}}$}	(s1)
(s1)
  edge node[sloped, anchor=center, above] {$gv_{\voterno,\prop{a}}$} (s2)
  edge node[sloped, anchor=center, above] {$ng_\voterno$} (s3)
(s2)
%  edge [bend left=60] node [sloped, anchor=center, above] {$repeat_\voterno$} (s0)
  edge node [left,near end] {$stop_\voterno$} (s4)
(s3)
%  edge node [sloped, anchor=center, above] {$repeat_\voterno$} (s0)
  edge node [left,near start] {$stop_\voterno$} (s4)
(s4)
  edge [loop left] node {} (s4)
%(s5)
%  edge [loop left] node {} (s5);
(s0)
  edge node[sloped, anchor=center, above] {$vote_{\voterno,\prop{b}}$}	(s1bis)
(s1bis)
  edge node[sloped, anchor=center, above] {$gv_{\voterno,\prop{b}}$} (s2bis)
  edge node[sloped, anchor=center, above] {$ng_\voterno$} (s3bis)
(s2bis)
%  edge [bend right=60] node [sloped, anchor=center, above] {$repeat_\voterno$} (s0)
  edge node [right,near end] {$stop_\voterno$} (s4bis)
(s3bis)
%  edge node [sloped, anchor=center, above] {$repeat_\voterno$} (s0)
  edge node [right,near start] {$stop_\voterno$} (s4bis)
(s4bis)
  edge [loop right] node {} (s4bis);

